ZeroSumEval: An Extensible Framework For Scaling LLM Evaluation with Inter-Model Competition

We introduce ZeroSumEval, a dynamic, competition-based, and evolving evaluation framework for Large Language Models (LLMs) that leverages competitive games. ZeroSumEval encompasses a diverse suite of games, including security challenges (Capture the Flag), classic board games (chess), and knowledge tests (MathQuiz). These games are designed to evaluate a range of capabilities such as strategic reasoning, planning, knowledge application, safety, and adaptability. Building upon recent studies that highlight the effectiveness of game-based evaluations for LLMs, ZeroSumEval enhances these approaches by providing a standardized and extensible framework for easily implementing games and leverages DSPy to provide a better abstraction for LLM player strategies.

==> figures/main_figure.tex <==
\begin{tikzpicture}[
    box/.style={draw, rectangle, rounded corners, minimum width=2.5cm, minimum height=1cm, fill=gray!20, text centered},
    process/.style={draw, rectangle, rounded corners, minimum width=2.5cm, minimum height=1cm, fill=red!20, text centered},
    optimization/.style={draw, rectangle, rounded corners, minimum width=2cm, minimum height=1cm, fill=blue!10, text centered},
    innerbox/.style={draw, rectangle, minimum width=1.2cm, minimum height=0.5cm, text centered},
    arrow/.style={->, thick},
    textblock/.style={rectangle, text centered}
]

% Leftmost ZSE Games Box
\node[draw, rectangle, rounded corners, minimum width=2.8cm, minimum height=5cm, fill=red!10] (zse) at (-4, 0) {};
\node[textblock] at (-4, 2) {ZSE Games};
\node[box] at (-4, 1) {Chess};
\node[box] at (-4, 0) {PyJail};
\node at (-4, -2) {...};

% Chess Leaderboard Box
\node[draw, rectangle, rounded corners, minimum width=4cm, minimum height=5cm, fill=blue!10] (leaderboard) at (0, 0) {};
\node[textblock] at (0, 2) {Chess Leaderboard};
\node[draw, rectangle, minimum width=2.8cm, minimum height=2.5cm, fill=blue!5] (leaderboard_inner) at (0, 0) {};
\node at (-1, 0.75) {$M_1$};
\node at (-1, 0.25) {$M_2$};
\node at (-1, -0.25) {$\vdots$};
\node at (-1, -0.75) {$M_n$};
\node at (1, 0.75) {$E_1$};
\node at (1, 0.25) {$E_2$};
\node at (1, -0.25) {$\vdots$};
\node at (1, -0.75) {$E_n$};

% Round Robin Box
\node[draw, rectangle, rounded corners, minimum width=3cm, minimum height=1.5cm, fill=gray!20] (roundrobin) at (3, 0) {Round Robin \\ Match $i$ \\ $M_x$ vs $M_y$};

% Chess Logic Box
\node[process, right=2cm of roundrobin] (logic) {Chess Logic};

% Optimization Boxes
\node[optimization, above=0.5cm of logic] (optA) {Strategy A};
\node[optimization, below=0.5cm of logic] (optB) {Strategy B};

% Winner Box
\node[draw, rectangle, rounded corners, minimum width=3cm, minimum height=2.5cm, fill=red!10] (winner) at (8, 0) {};
\node[box] at (8, 0.75) {$e_x++$};
\node[textblock] at (8, 0) {$M_x$ Wins!};
\node[box] at (8, -0.75) {$e_y--$};

% Arrows
\draw[arrow] (zse) -- (leaderboard);
\draw[arrow] (leaderboard) -- node[above] {} (roundrobin);
\draw[arrow] (roundrobin) -- (logic);
\draw[arrow] (optA) -- (logic);
\draw[arrow] (optB) -- (logic);
\draw[arrow] (logic) -- (winner);

\end{tikzpicture}

==> figures/ver_figure.tex <==
\begin{wrapfigure}[24]{R}{0.5\linewidth}
\vspace{-1em}
    \begin{center}
    \begin{tikzpicture}[
        box/.style={rectangle, draw, rounded corners, fill=blue!10, drop shadow, minimum height=0.8cm, minimum width=2.8cm, align=center},
        boxllm/.style={rectangle, draw, rounded corners, fill=green!10, drop shadow, minimum height=0.8cm, minimum width=2.8cm, align=center},
        actor/.style={circle, fill=white!10, draw, drop shadow, minimum size=0.8cm},
        arrow/.style={-Stealth, thick, draw=black!80},
        node distance=1cm and 2cm
    ]

    % Actors
    \node[actor, label=above:{\textbf{Manager}}] (manager) at (-2, 0.5) {M};
    \node[actor, label=above:{\textbf{Generator}}] (generator) at (2, 0.5) {G};

    % Nodes for Manager
    \node[box, below=of manager] (generate) {Generate Target};
    \node[box, below=of generate] (verify) {Verification};
    \node[box, below=of verify] (match) {Match Target?};

    % Nodes for Generator
    \node[boxllm, below=of generator] (genModel) {Receive Target};
    \node[boxllm, below=of genModel] (output) {Generate Challenge};
    \node[boxllm, below=of output] (clear) {Solve Challenge};

    % Arrows between Manager and Generator
    \draw[arrow] (generate) -- (genModel) node[midway, above, font=\small] {Target};
    \draw[arrow] (genModel) -- (output);
    \draw[arrow] (output) -- (verify);
    \draw[arrow] (verify) -- (clear) node[midway, above, sloped, font=\small] {Clear};
    \draw[arrow] (clear) -- (match);

    % Dashed line separating roles
    \draw[dashed, thick, dash pattern=on 5pt off 10pt] (0, 1) -- (0, -5.5) node[midway, right, fill=white, inner sep=1pt] {};


    % Labels for clarity
    \node[above=0.2cm of manager] (manager_label) {};
    \node[above=0.2cm of generator] (generator_label) {};

    \end{tikzpicture}
    \end{center}
    \caption{State diagram of the verification process involving the Game Manager and the Generator. Blue boxes indicate deterministic steps and green boxes indicate steps involving the model.}
    \label{fig:state-diagram-verification}
\end{wrapfigure}

==> sections/30_methodology.tex <==
% - List the models tested and the reasoning behind that choice
% - Conduct multiple tournament runs per setup to ensure stability
% - Observe the difference in rankings between with prompt optimization and without prompt optimization
% - Do all runs with the dspy.ChainOfThought module, imploring future work to test the  effects different prompting strategies make on the rankings

In this section, we describe the technical details of \ZSEVAL{} including design choices, the importance of automatic prompt optimization, and game selection/categorization. At its core, \ZSEVAL{} provides controlled environments to observe models competing against each other to win competitive games. In particular, ZSE controls (i) the role and information each model has access to at any point in the simulation and (ii) the data models can use to optimize/modify their own prompts. 

\subsection{Capabilities}

The games within ZSE are designed to evaluate specific capabilities in a controlled environment:

\paragraph{Reasoning} Board games and cybersecurity scenarios require models to perform complex, multi-step reasoning. They test the models' ability to process information, predict outcomes, and formulate strategies in dynamically changing environments.

\paragraph{Planning} Board games also involve long-term strategy, requiring models to anticipate the consequences of their actions several moves ahead. This assesses the model’s foresight, adaptability, and capacity for nuanced decision-making.

\paragraph{Knowledge Application} Models must recall and apply mathematical knowledge to solve problems in question answering type games. This setup provides a direct assessment of the models' ability to retrieve, interpret, and implement factual information in structured problem-solving.

\paragraph{Creativity} Models successful at cybersecurity type games must exhibit creativity to successfully create secure environments and break them.

\subsection{Game Design}

\ZSEVAL{} supports an expanding suite of game types designed to test the aspects of LLM performance described above. The mix we showcase includes both well-known and established games, such as chess, as well as more special-purpose games (e.g. MathQuiz). 
For completeness and reproducibility, we describe the implementations of MathQuiz and PyJail. The following set of games are selected to encompass a range of cognitive capabilities, including strategic reasoning, planning, knowledge application, and creativity:

\begin{wrapfigure}[25]{R}{0.5\linewidth}
    \vspace{-2em}
  \begin{center}
    \includegraphics[width=0.95\linewidth]{figures/final/correct_plans.pdf}
  \end{center}
  \caption{The effect of prompt optimization on the proportion of correct moves. Moves are classified as correct if the evaluation, as determined by Stockfish 17 \citep{stockfish} with depth 15, does not decrease by more than 0.3 points (pawn equivalent). Models react differently to prompts and have varying prompt optimization abilities.}
  \label{fig:correct_plans}
\end{wrapfigure}

\paragraph{Board Games (Chess)} Classic board games like chess serve as a benchmark for strategic reasoning and long-term planning. They require models to engage in multi-step thinking, manage trade-offs, and foresee opponent moves. This category is instrumental in evaluating a model's ability to plan several moves ahead, adapt its strategies, and make complex decisions under uncertainty\footnote{Chess has a rich history as a testbed for strategy and planning. See \url{https://github.com/carlini/chess-llm} and \url{https://huggingface.co/spaces/mlabonne/chessllm} for examples of LLMs playing chess.}.

\paragraph{Question-Answer Games (MathQuiz)} These games are constructed to measure models' knowledge recall and logical reasoning abilities. MathQuiz, for instance, challenges models to both create and answer arithmetic and mathematical questions, assessing their understanding of mathematical concepts, computational accuracy, and step-by-step problem-solving skills. Our implementation of MathQuiz tasks a teacher player to create a challenging math problem and prove that the problem is valid and solvable. A student player then attempts to answer the generated math problem. The student wins the game by answering the question correctly or if the teacher fails to create a valid question.

% \paragraph{Conversational Games (Gandalf)} Designed to assess models' creative capabilities and susceptability/resistance to jailbreaking, Gandalf engages LLMs in scenarios where one player attempts to break the conditioning of another. In this game, a sentinel player is tasked to keep a randomly generated passphrase secret while conversing with an infiltrator player. The infiltrator wins if the passphrase is revealed in the conversation and the sentinel wins if the conversation exceeds a maximum number of turns. CITE CYBERSECEVAL/LLAMA3.1

\paragraph{Cybersecurity Games (PyJail)} PyJail involves python ``capture the flag'' cybersecurity challenges, targeting the model's ability to create puzzles and interact with a restricted python environment to strategize solutions. The PyJail game is structured into three stages. The first statically parses a player generated PyJail program to provide feedback on the syntax and semantic structure. Given validity, the challenge code is inserted into the environment, and the same player model must commit a solution that is tested dynamically to prove the challenge's feasibility. A unique flag is stored in the target variable at runtime, which prevents any trivial method to cheat the challenge. The second player will complete the same step, provided a restricted view of the environment and limited context. The game ends if first player is unable to create a valid challenge or the flag is retrieved by the attacker.

% TODO: this figure looks very weird in this template. @Haidar any easy way to fix this?
\begin{wrapfigure}[24]{R}{0.5\linewidth}
\vspace{-1em}
    \begin{center}
    \begin{tikzpicture}[
        box/.style={rectangle, draw, rounded corners, fill=blue!10, drop shadow, minimum height=0.8cm, minimum width=2.8cm, align=center},
        boxllm/.style={rectangle, draw, rounded corners, fill=green!10, drop shadow, minimum height=0.8cm, minimum width=2.8cm, align=center},
        actor/.style={circle, fill=white!10, draw, drop shadow, minimum size=0.8cm},
        arrow/.style={-Stealth, thick, draw=black!80},
        node distance=1cm and 2cm
    ]

    % Actors
    \node[actor, label=above:{\textbf{Manager}}] (manager) at (-2, 0.5) {M};
    \node[actor, label=above:{\textbf{Generator}}] (generator) at (2, 0.5) {G};

    % Nodes for Manager
    \node[box, below=of manager] (generate) {Generate Target};
    \node[box, below=of generate] (verify) {Verification};
    \node[box, below=of verify] (match) {Match Target?};

    % Nodes for Generator
    \node[boxllm, below=of generator] (genModel) {Receive Target};
    \node[boxllm, below=of genModel] (output) {Generate Challenge};
    \node[boxllm, below=of output] (clear) {Solve Challenge};

    % Arrows between Manager and Generator
    \draw[arrow] (generate) -- (genModel) node[midway, above, font=\small] {Target};
    \draw[arrow] (genModel) -- (output);
    \draw[arrow] (output) -- (verify);
    \draw[arrow] (verify) -- (clear) node[midway, above, sloped, font=\small] {Clear};
    \draw[arrow] (clear) -- (match);

    % Dashed line separating roles
    \draw[dashed, thick, dash pattern=on 5pt off 10pt] (0, 1) -- (0, -5.5) node[midway, right, fill=white, inner sep=1pt] {};


    % Labels for clarity
    \node[above=0.2cm of manager] (manager_label) {};
    \node[above=0.2cm of generator] (generator_label) {};

    \end{tikzpicture}
    \end{center}
    \caption{State diagram of the verification process involving the Game Manager and the Generator. Blue boxes indicate deterministic steps and green boxes indicate steps involving the model.}
    \label{fig:state-diagram-verification}
\end{wrapfigure}

\subsection{Scalable Verification}

The MathQuiz and PyJail games require competing models to generate complex challenge environments and solutions. Since verification of the knowledge-based challenges by a human in the loop is not scalable, we design a method to verify model output using an automated manager in a two-fold generation and verification process. This is accomplished by defining a target outcome (e.g., the answer to a math question or a CTF flag) as the basis for verifying generated input, and regulating the model context at each stage.

The exact process (illustrated in \Cref{fig:state-diagram-verification}) is outlined as follows:

(i) The generator model receives a target and attempts to output a valid challenge that resolves to the specific target.

(ii) In the verification step, the manager restricts the model's context to ensure no direct access to the target, and asks the generator model to solve the previously generated challenge.

(iii) If the manager determines the verification is successful (by matching the target with the generator's solution), the game proceeds. Otherwise, the generator model is deemed to have failed to generate a valid challenge.

This method ensures the generated challenge environment is valid and a solution is proven possible by the generator. The design also correctly penalizes models that directly generate memorized questions as it is likely to have been memorized by other models, thereby encouraging models to create challenging and novel questions. Finally, the scalability of the evaluation is preserved as the capabilities of models scale.

% IF THERE IS SPACE I WILL ADD THE PROBABILISTIC ARGUMENT FOR WHY THIS MAKES SENSE

\subsection{Automatic Prompting}

Automatic prompting is an essential component of the \ZSEVAL{} framework for several reasons. First, it allows models to learn to play new games through self-optimization, demonstrating their ability to adapt to different scenarios without human intervention. Second, it removes the human element in prompt engineering, thereby reducing biases and variations introduced by manual prompt construction \citep{zheng2024largelanguagemodelsrobust,pezeshkpour2023largelanguagemodelssensitivity,alzahrani2024benchmarks}. Third, automatic prompting serves as a measure of a model's ability to self-improve at inference time, providing insight into its adaptability and strategic reasoning skills.

We leverage the DSPy \citep{khattab2023dspy} approach to implement automatic prompt optimization in our framework. DSPy allows models to autonomously explore and select optimal prompts based on the current game context, dynamically adjusting strategies to maximize performance. We also make use of DSPy Assertions \citep{singhvi2024dspyassertionscomputationalconstraints} to simulate interactivity between the models and the game environment by allowing a number of retries (with feedback from the game) when the model makes an invalid move. Although we find DSPy has the flexibility and generalizability to support various models and games, \ZSEVAL{} supports alternative automatic prompt optimization techniques if required.

Through prompt optimization, models can develop improved strategies as they encounter diverse game scenarios. For example, in a chess game, models equipped with optimized prompting demonstrated a higher proportion of correct moves compared to their counterparts using default prompts \Cref{fig:correct_plans}. This not only reveals the models' enhanced strategic reasoning but also emphasizes the significance of prompt optimization in robust performance evaluation.

By incorporating automatic prompting, \ZSEVAL{} addresses benchmark sensitivity. The prompt optimization integrates game validation mechanisms into the optimization process, allowing models to observe tangible outcomes and refine their prompt strategies. Consequently, this mitigates the variations in performance due to prompt sensitivity, leading to a more consistent and reliable evaluation of model capabilities.

\paragraph{Datasets and Optimizers} To perform the automatic prompt optimization process, models require examples of gameplay (inputs and outputs) and prompt optimizers. We create standard datasets manually for each game available to all models for the optimization. The available datasets are described in \Cref{tab:datasets}. Through DSPy, \ZSEVAL{} supports multiple types of optimizers. In this work, we focus on (i) BootstrapFewShot (ii) BootstrapFewShotRandomSearch \citep{khattab2023dspy} and (iii) MIPROv2 \citep{opsahlong2024miprov2}.

% \begin{table}[htbp]
% \centering
% \small
% \begin{tabular}{lll}
% \toprule
% \textbf{Dataset} & \textbf{Source} & \textbf{Description} \\ \midrule
% chess\_stockfish & conacts/stockfish\_dataset\footnote{\url{https://huggingface.co/datasets/conacts/stockfish_dataset}} & stockfish vs stockfish games \\ 
% chess\_puzzles & \citep{schwarzschild2021datasets} &  chess puzzles. \\ 
% mathquiz\_gsm8k & \citep{gsm8k} & grade school level math QA \\ 
% mathquiz\_hendrycks\_math & \citep{hendrycksmath} & advanced math QA \\ 
% % gandalf\_cyberseceval & XXX & CITE & A dataset of jailbreak illustrations. \\ 
% pyjail\_ctf\_llm & \citep{shao2024nyuctfdatasetscalable} & Pyjail style Capture The Flags (CTFs). \\ \bottomrule
% \end{tabular}
% \caption{Overview of datasets used in the evaluation framework.}
% \label{tab:datasets}
% \end{table}


An interesting direction out of the scope of this work is enabling models to learn games via self-play. This would reduce manual effort needed to create new games for \ZSEVAL{} and measure a model's ability to effectively explore a space without supervision.  

\subsection{Ratings}

\ZSEVAL{}{} utilizes an easily computable rating system derived from the outcomes of competitive games between models. Each model receives a rating based on its win-loss record over multiple games, allowing for a rapid and scalable oversight of model capabilities. This framework seamlessly incorporates new games, providing continuous and dynamic evaluation as models improve.

Following recent suggestions for LLM rating systems by \citet{boubdir2023elouncoveredrobustnessbest,eloarena2023}, we employ the Bradley-Terry (BT) rating system, an alternative to the Elo system, to rate models. The BT model is permutation-invariant and assumes a fixed win rate for each model pair, maximizing the likelihood of observed outcomes \citep{bradleyterryrank}. This choice is more suitable than the traditional Elo system, which was designed for human chess players with varying skill levels, whereas LLMs have fixed skill levels defined by their weights \citep{elo}.

\ZSEVAL{}'s rating system facilitates analysis of model behaviors. It allows us to observe not only the relative strategic planning capabilities of models but also their capacity for self-improvement through prompt optimization. For instance, analysis of models’ gameplay strategies in chess revealed that prompt-optimized models allocate more reasoning words in their decision-making process, suggesting a deeper level of planning (\Cref{fig:cot_words}). %Similarly, models that engaged in prompt optimization showed a reduced distribution of negative evaluation deltas, indicating more effective decision-making (\Cref{fig:stockfish_delta}).


==> sections/50_experiments.tex <==
% - Stability: 5 runs without optimization
% - Prompt Sensitivity: 5 runs with optimization
% - Absolute vs Relative: Compare to SOTA benchmark rankings

% Experimental setup

% - models tested

% - game settings

% - DSPy modules and optimizers

% - Matchings (round robin)

% - compiling tournament data

In this section, we describe the experiments to demonstrate the effectiveness of the \ZSEVAL{} as a dynamic leaderboard. We also design experiments to evaluate the effect of prompt optimization on the performance of various large language models (LLMs) under various simulations. 

\subsection{Model Selection and Experimental Setup}

We select four models of varying sizes and capabilities for this study: GPT-4o, Claude 3.5 Sonnet, LLaMA 3.1-70B-Instruct, and Mistral-Large. These models represent a range of architectures and training scales, providing a diverse set for evaluating the generalizability of the \ZSEVAL{} framework.

The experiments involve running a multiple round-robin tournaments to simulate competitive gameplay among the model (50-100 games per experiment). In addition to measuring model performance on the games in the \ZSEVAL{} suite, we also examine how the models' performance changes with different prompt optimization techniques. Each tournament round involves all possible match permutations between model variants, after which the models' ratings are calculated using the Bradley-Terry model \citep{bradleyterryrank}. The primary goal of this ablation study is to assess each model's responsiveness to the optimization process and to identify resulting behavioral changes.

For the automatic prompt optimization, we utilize three optimizers commonly used in DSPy: BootstrapFewshot (BSFS), BootstrapFewshotWithRandomSearch (BSFSRS), and MIPROv2, targeting the ChainOfThought module in DSPy.

\subsection{Games for Analysis}

Although \ZSEVAL{} supports a range of games for assessing different capabilities, our detailed set of experiments focus primarily on Chess to analyze the models' planning abilities. This decision is motivated by the interpretability of Chess gameplay and its complexity, which provides an ideal testbed for assessing strategic reasoning and decision-making.

==> tables/model_versions.tex <==
% \begin{table}[ht]
%     \caption{Exact model versions used in our evaluations.}
%     \centering
%     \begin{tabular}{ll}
%         \toprule
%         Model & Version \\
%         \midrule
%         GPT-4o & \texttt{gpt-4o-2024-08-06} \\
%         Claude 3.5 Sonnet & \texttt{claude-3-5-sonnet-20240620} \\
%         Mistral-Large & \href{https://huggingface.co/mistralai/Mistral-Large-Instruct-2407}{\texttt{mistralai/Mistral-Large-Instruct-2407}} \\
%         Llama 3.1 70B & \href{https://huggingface.co/meta-llama/Meta-Llama-3.1-70B-Instruct}{\texttt{meta-llama/Meta-Llama-3.1-70B-Instruct}} \\
%         \bottomrule
%     \end{tabular}
%     \label{table:model_versions}
% \end{table}

